Measurement of the radiative decay of polarized muons in the MEG experiment

We studied the radiative muon decay $\mu^+ \to e^+\nu\bar{\nu}\gamma$ by using for the first time an almost fully polarized muon source. We identified a large sample (~13000) of these decays in a total sample of 1.8x10^14 positive muon decays collected in the MEG experiment in the years 2009--2010 and measured the branching ratio B($\mu^+ \to e^+\nu\bar{\nu}\gamma$) = (6.03+-0.14(stat.)+-0.53(sys.))x10^-8 for E_e > 45 MeV and E_{\gamma} > 40 MeV, consistent with the Standard Model prediction. The precise measurement of this decay mode provides a basic tool for the timing calibration, a normalization channel, and a strong quality check of the complete MEG experiment in the search for $\mu^+ \to e^+\gamma$ process.

==> institute_INFNComb-epjc.tex <==
\newcommand*{\INFNPi}{INFN Sezione di Pisa$^{a}$; Dipartimento di Fisica$^{b}$ dell'Universit\`a, Largo B.~Pontecorvo~3, 56127 Pisa, Italy}
\newcommand*{\ScuolaPi}{Scuola Normale Superiore, Piazza dei Cvalieri 7, 56127 Pisa, Italy}
%\newcommand*{\INFNPi}{INFN Sezione di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}
%\newcommand*{\UniPi}{Dipartimento di Fisica, Universit\`a di Pisa, Largo B. Pontecorvo 3, 56127 Pisa, Italy}

\newcommand*{\INFNGe}{INFN Sezione di Genova$^{a}$; Dipartimento di Fisica$^{b}$ dell'Universit\`a, Via Dodecaneso 33, 16146 Genova, Italy}
%\newcommand*{\INFNGe}{INFN Sezione di Genova, Via Dodecaneso 33, 16146 Genova, Italy}
%\newcommand*{\UniGe}{Dipartimento di Fisica, Universit\`a degli Studi di Genova, Via Dodecaneso 33, 16146 Genova, Italy}

\newcommand*{\INFNPv}{INFN Sezione di Pavia$^{a}$; Dipartimento di Fisica$^{b}$ dell'Universit\`a, Via Bassi 6, 27100 Pavia, Italy}
%\newcommand*{\INFNPv}{INFN Sezione di Pavia, Via Bassi 6, 27100 Pavia, Italy}
%\newcommand*{\UniPv}{Dipartimento di Fisica, Universit\`a di Pavia, Via Bassi 6, 27100 Pavia, Italy}

\newcommand*{\INFNRm}{INFN Sezione di Roma$^{a}$; Dipartimento di Fisica$^{b}$ dell'Universit\`a ``Sapienza'', Piazzale A.~Moro, 00185 Roma, Italy}
%\newcommand*{\INFNRm}{INFN Sezione di Roma, Piazzale A.~Moro, 00185 Roma, Italy}
%\newcommand*{\UniRm}{Dipartimento di Fisica, Universit\`a  di Roma \lq\lq{}Sapienza\rq\rq{}, Piazzale A.~Moro, 00185 Roma, Italy}

\newcommand*{\INFNLe}{INFN Sezione di Lecce$^{a}$; Dipartimento di Matematica e Fisica$^{b}$ dell'Universit\`a del Salento, Via per Arnesano, 73100 Lecce, Italy}
%\newcommand*{\INFNLe}{INFN Sezione di Lecce, Via per Arnesano, 73100 Lecce, Italy}
%\newcommand*{\UniLe}{Dipartimento di Matematica e Fisica, Universit\`a  del Salento, Via per Arnesano, 73100 Lecce, Italy}

\newcommand*{\ICEPP} {ICEPP, The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, Tokyo 113-0033, Japan }
\newcommand*{\UCI}   {University of California, Irvine, CA 92697, USA}
\newcommand*{\KEK}   {KEK, High Energy Accelerator Research Organization, 1-1 Oho, Tsukuba, Ibaraki 305-0801, Japan}
\newcommand*{\PSI}   {Paul Scherrer Institut PSI, CH-5232 Villigen, Switzerland}
\newcommand*{\Waseda}{Research Institute for Science and Engineering, Waseda~University, 3-4-1 Okubo, Shinjuku-ku, Tokyo 169-8555, Japan}
\newcommand*{\BINP}  {Budker Institute of Nuclear Physics of Siberian Branch of Russian Academy of Sciences, 630090 Novosibirsk, Russia}
\newcommand*{\JINR}  {Joint Institute for Nuclear Research, 141980 Dubna, Russia}
\newcommand*{\ETHZ}  {Swiss Federal Institute of Technology ETH, CH-8093 Z\" urich, Switzerland}
\newcommand*{\NOVS}  {Novosibirsk State University, 630090 Novosibirsk, Russia}
\newcommand*{\NOVST}  {Novosibirsk State Technical University, 630092 Novosibirsk, Russia}


